LatentMimic: Terrain-Adaptive Locomotion via Latent Space Imitation

Developing natural and diverse locomotion controllers for quadruped robots that can adapt to complex terrains while preserving motion style remains a significant challenge. Existing imitation-based methods face a fundamental optimization trade-off: strict adherence to motion capture (mocap) references penalizes the geometric deviations required for terrain adaptability, whereas terrain-centric policies often compromise stylistic fidelity. We introduce LatentMimic, a novel locomotion learning framework that decouples stylistic fidelity from geometric constraints. By minimizing the marginal latent divergence between the policy's state-action distribution and a learned mocap prior, our approach provides a conditional relaxation of rigid pose-tracking objectives. This formulation preserves gait topology while permitting independent end-effector adaptations for irregular terrains. We further introduce a terrain adaptation module with a dynamic replay buffer to resolve the policy's distribution shifts across different terrains. We validate our method across four locomotion styles and four terrains, demonstrating that LatentMimic enables effective terrain-adaptive locomotion, achieving higher terrain traversal success rates than state-of-the-art motion-tracking methods while maintaining high stylistic fidelity.

==> speak.tex <==
1. Title:
2. Background:
Learning locomotion via motion imitation has become a popular solution for developing legged robot controllers. 
3. Background:
However, the motion capture data is usually limited in its modality, posing challenges in generalizing the learned locomotion styles to diverse terrains. For instance, the target walking motion may step into stairs instead of on the stair.
4. Methodology:
To address these limitations, we propose a two-stage learning framework. The framework comprises two modules:
1) A latent mimic learning module that employs a single mimic reward to train a style locomotion policy in latent space.
2) A terrain adaptation module that facilitates the transfer of locomotion styles to various terrains.
5. Methodology:
In the latent space imitation learning phase, we introduce a Latent Prior Module that encodes both the target motion and simulated motion into latent space. Subsequently, a single latent mimic reward is utilized to train the locomotion styles on flat terrain.
6. Methodology:
In the terrain adaptation learning phase, we introduce a terrain adaptation replay buffer that samples high-performance frames from diverse levels of terrains. These frames are utilized to refine the motion predictor, enabling the generation of target frames in terrain adaptation learning.
7. Results:
We demonstrate the effectiveness of our latent mimic learning approach with four distinct locomotion styles: pace, trot, pace backward, and trot backward. The pace and trot locomotion styles are retargeted from motion capture data, while the backward styles are generated by reversing the motion capture data. The result shows that the target motion could be learned with a single latent mimic reward without multiple complex rewards or a discriminator in AMP.
8. Results:
We also present the terrain adaptation results for four locomotion styles on stairs, noise, waves, and uneven terrain. Our experiments demonstrate that our method can successfully navigate higher-level terrains while preserving the locomotion styles compared to previous approaches.

8. Final: Please see our locomotion results in the following video.     
